Same Coverage, Less Bloat: Accelerating Binary-only Fuzzing with Coverage-preserving Coverage-guided Tracing

Coverage-guided fuzzing's aggressive, high-volume testing has helped reveal tens of thousands of software security flaws. While executing billions of test cases mandates fast code coverage tracing, the nature of binary-only targets leads to reduced tracing performance. A recent advancement in binary fuzzing performance is Coverage-guided Tracing (CGT), which brings orders-of-magnitude gains in throughput by restricting the expense of coverage tracing to only when new coverage is guaranteed. Unfortunately, CGT suits only a basic block coverage granularity -- yet most fuzzers require finer-grain coverage metrics: edge coverage and hit counts. It is this limitation which prohibits nearly all of today's state-of-the-art fuzzers from attaining the performance benefits of CGT. This paper tackles the challenges of adapting CGT to fuzzing's most ubiquitous coverage metrics. We introduce and implement a suite of enhancements that expand CGT's introspection to fuzzing's most common code coverage metrics, while maintaining its orders-of-magnitude speedup over conventional always-on coverage tracing. We evaluate their trade-offs with respect to fuzzing performance and effectiveness across 12 diverse real-world binaries (8 open- and 4 closed-source). On average, our coverage-preserving CGT attains near-identical speed to the present block-coverage-only CGT, UnTracer; and outperforms leading binary- and source-level coverage tracers QEMU, Dyninst, RetroWrite, and AFL-Clang by 2-24x, finding more bugs in less time.

==> figures/tab_hybrid.tex <==
\begin{table*}[!h]
\scriptsize   
%
    \centering
    
    %\small
    %\rowcolors{2}{gray!25}{white}
    \begin{tabular}[b]{p{1.55cm} | cccc | cccc cccc }
        \specialrule{.1em}{0em}{0em} 
        \hline
        
        \mystrut
        \multirow{3}{*}{\textbf{Binary}} & 
        \multicolumn{4}{c|}{{\notsosmall{vs. \emph{Coverage-guided Tracing}}}} &
        \multicolumn{8}{c}{{\notsosmall{vs. Binary- and Source-level \emph{Conventional Tracing}}}} \\

        %\cline{2-11}
        \mystrut 
        &
        \multicolumn{4}{c|}{\cellcolor{white}\textbf{\scriptsize{QSYM-\platname\phantom{} / QSYM-UnTracer}}} &
        \multicolumn{4}{c}{\cellcolor{white}\textbf{\scriptsize{QSYM-\platname\phantom{} / QSYM-QEMU}}} &
        \multicolumn{4}{c}{\cellcolor{white}\textbf{\scriptsize{QSYM-\platname\phantom{} / QSYM-Clang}}} \\
        
        & 
        \notsotiny{{{Rel. Perf}}} & 
        \notsotiny{MWU } &        
        \notsotiny{{{Rel. Bugs}}} & 
        \notsotiny{MWU } &
        \notsotiny{{{Rel. Perf}}} &  
        \notsotiny{MWU } &
        \notsotiny{{{Rel. Bugs}}} & 
        \notsotiny{MWU } &
        \notsotiny{{{Rel. Perf}}} & 
        \notsotiny{MWU } &
        \notsotiny{{{Rel. Bugs}}} &
        \notsotiny{MWU } \\
 
        \hline
        \hline
        \rowcolor{gray!10}\texttt{jasper} & 
        0.99 & 0.435 & 1.39 & \textbf{0.003} &
        \xmarktab & \xmarktab & \xmarktab & \xmarktab &
        2.15 & \textbf{0.003} & 1.00 & 0.485 \\
        
        \texttt{mjs} & 
        0.87 & 0.020 & 0.98 & 0.103 &
        12.41 & \textbf{$<$0.001} & 4.18 & \textbf{$<$0.001} &
        4.13 & \textbf{$<$0.001} & 1.87 & \textbf{$<$0.001} \\
                
        \rowcolor{gray!10}\texttt{nasm} & 
        2.18 & \textbf{$<$0.001} & 1.02 & 0.269 &
        14.51 & \textbf{$<$0.001} & 15.55 & \textbf{$<$0.001} &
        1.33 & \textbf{$<$0.001} & 1.32 & \textbf{$<$0.001} \\
                
        \texttt{sfconvert} & 
        0.91 & 0.010 & 1.12 & \textbf{0.013} &
        \xmarktab & \xmarktab & \xmarktab & \xmarktab &
        2.35 & \textbf{$<$0.001} & 1.05 & 0.251 \\
                
         \rowcolor{gray!10}\texttt{tcpdump} & 
        1.00 & 0.068 & 0.97 & 0.122 &
        1.76 & \textbf{$<$0.001} & 1.39 & \textbf{$<$0.001} &
        1.01 & 0.448 & 1.14 & 0.211 \\
        
       \texttt{unrtf} & 
        1.06 & 0.346 & 1.31 & \textbf{$<$0.001} &
        4.48 & \textbf{$<$0.001} & 1.20 & \textbf{$<$0.001} &
        2.33 & \textbf{$<$0.001} & 1.45 & \textbf{$<$0.001} \\
                
        \rowcolor{gray!10}\texttt{yara} & 
        0.76 & 0.047 & 0.87 & 0.023 &
        11.80 & \textbf{$<$0.001} & 1.72 & \textbf{$<$0.001} &
        4.56 & \textbf{$<$0.001} & 1.41 & \textbf{$<$0.001} \\
                
        %\hline
        
        \texttt{lzturbo} & 
        0.86 & 0.118 & \xmarktab  & \xmarktab  &
        9.45 & \textbf{$<$0.001} & \xmarktab  & \xmarktab  &
        \xmarktab & \xmarktab & \xmarktab & \xmarktab \\
         
        \rowcolor{gray!10}\texttt{pngout} & 
        0.54 & $<$0.001 & 1.14 & \textbf{$<$0.001} &
        16.14 & \textbf{$<$0.001} & 2.18 & \textbf{$<$0.001} &
        \xmarktab & \xmarktab & \xmarktab & \xmarktab \\

        \texttt{rar} & 
        0.83 & 0.006 & \xmarktab & \xmarktab & 
        7.29 & \textbf{$<$0.001} & \xmarktab & \xmarktab & 
        \xmarktab & \xmarktab & \xmarktab & \xmarktab \\         
        

        \rowcolor{gray!10}\texttt{unrar} & 
        0.79 & 0.002 & 1.25 & 0.104 &
        3.13 & \textbf{$<$0.001} & 0.38 & $<$0.001 &
        \xmarktab & \xmarktab & \xmarktab & \xmarktab \\
         
        \hline

                
        \multicolumn{1}{l|}{\scriptsize{\textbf{Mean Increase}}} & 
        \textbf{-2\%} &  & \textbf{+12\%} &  &
        \textbf{+800\%} &  & \textbf{+280\%} &  &
        \textbf{+155\%} &  & \textbf{+32\%} &  \\
   

    \end{tabular}
    \vspace{-0.0cm}
    \caption{\textbf{QSYM-\platname's mean throughput and bugs} relative to QSYM-UnTracer, QSYM-QEMU, QSYM-Clang. We omit \texttt{lzturbo} and \texttt{rar} as no fuzzing trials trigger any crashes for them, and \texttt{sam2p} as it fails on all QSYM configurations. \emph{\xmarktab} = the competing tracer is incompatible with the respective benchmark and hence omitted. Statistically significant improvements in for \platname (i.e., Mann-Whitney U test $p < 0.05$) are \textbf{bolded}. }
    \label{tab:hybrid}
\vspace{-0.4cm}
\hrulefill{}
%\vspace{0.2cm}
\end{table*}
